Isogeometric analysis of linear free-surface potential flow

This paper presents a novel variational formulation to simulate linear free-surface flow. The variational formulation is suitable for higher-order finite elements and higher-order and higher-continuity shape functions as employed in Isogeometric Analysis (IGA). The novel formulation combines the interior and free-surface problems in one monolithic formulation. This leads to exact energy conservation and superior performance in terms of accuracy when compared to a traditional segregated formulation. This is confirmed by the numerical computation of traveling waves in a periodic domain and a three-dimensional sloshing problem. The isogeometric approach shows significant improved performance compared to traditional finite elements. Even on very coarse quadratic NURBS meshes the dispersion error is virtually absent.

==> figs/trace2_p1.tex <==

\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f3p1r1.pdf}
\caption{6 x 6 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f3p1r2.pdf}
\caption{12 x 12 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f3p1r3.pdf}
\caption{24 x 24 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f3p1r4.pdf}
\caption{48 x 48 mesh}
\end{subfigure}
\end{center}
\caption{Energy time trace for the segregated formulation with linear finite elements}
\label{fig:tracef3p1}
\end{figure}

\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f2p1r1.pdf}
\caption{6 x 6 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f2p1r2.pdf}
\caption{12 x 12 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f2p1r3.pdf}
\caption{24 x 24 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f2p1r4.pdf}
\caption{48 x 48 mesh}
\end{subfigure}
\end{center}
\caption{Energy time trace for segregated formulation with linear finite elements}
\label{fig:tracef2p1}
\end{figure}



==> figs/trace2_p2.tex <==


\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f3p2r0.pdf}
\caption{3 x 3 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f3p2r1.pdf}
\caption{6 x 6 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f3p2r2.pdf}
\caption{12 x 12 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f3p2r3.pdf}
\caption{24 x 24 mesh}
\end{subfigure}
\end{center}
\caption{Energy time trace for the segregated formulation with quadratic finite elements}
\label{fig:tracef3p2}
\end{figure}


\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f2p2r0.pdf}
\caption{3 x 3 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f2p2r1.pdf}
\caption{6 x 6 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f2p2r2.pdf}
\caption{12 x 12 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs/trace2_f2p2r3.pdf}
\caption{24 x 24 mesh}
\end{subfigure}
\end{center}
\caption{Energy time trace for the monolithic formulation with quadratic finite elements}
\label{fig:tracef2p2}
\end{figure}


==> figs3/trace2_p1.tex <==

\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f3p1r1.pdf}
\caption{6 x 6 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f3p1r2.pdf}
\caption{12 x 12 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f3p1r3.pdf}
\caption{24 x 24 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f3p1r4.pdf}
\caption{48 x 48 mesh}
\end{subfigure}
\end{center}
\caption{Energy time trace for the segregated formulation with linear finite elements}
\label{fig:tracef3p1}
\end{figure}

\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f2p1r1.pdf}
\caption{6 x 6 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f2p1r2.pdf}
\caption{12 x 12 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f2p1r3.pdf}
\caption{24 x 24 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f2p1r4.pdf}
\caption{48 x 48 mesh}
\end{subfigure}
\end{center}
\caption{Energy time trace for segregated formulation with linear finite elements}
\label{fig:tracef2p1}
\end{figure}



==> figs3/trace2_p2.tex <==


\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f3p2r0.pdf}
\caption{3 x 3 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f3p2r1.pdf}
\caption{6 x 6 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f3p2r2.pdf}
\caption{12 x 12 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f3p2r3.pdf}
\caption{24 x 24 mesh}
\end{subfigure}
\end{center}
\caption{Energy time trace for the segregated formulation with quadratic finite elements}
\label{fig:tracef3p2}
\end{figure}


\begin{figure}[!htb]
\begin{center}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f2p2r0.pdf}
\caption{3 x 3 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f2p2r1.pdf}
\caption{6 x 6 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f2p2r2.pdf}
\caption{12 x 12 mesh}
\end{subfigure}
\begin{subfigure}[b]{0.39\textwidth}
\centering
\includegraphics[width=\textwidth]{runs/figs3/trace2_f2p2r3.pdf}
\caption{24 x 24 mesh}
\end{subfigure}
\end{center}
\caption{Energy time trace for the monolithic formulation with quadratic finite elements}
\label{fig:tracef2p2}
\end{figure}

